AutoDetect: Towards a Unified Framework for Automated Weakness Detection in Large Language Models

Although Large Language Models (LLMs) are becoming increasingly powerful, they still exhibit significant but subtle weaknesses, such as mistakes in instruction-following or coding tasks. As these unexpected errors could lead to severe consequences in practical deployments, it is crucial to investigate the limitations within LLMs systematically. Traditional benchmarking approaches cannot thoroughly pinpoint specific model deficiencies, while manual inspections are costly and not scalable. In this paper, we introduce a unified framework, AutoDetect, to automatically expose weaknesses in LLMs across various tasks. Inspired by the educational assessment process that measures students' learning outcomes, AutoDetect consists of three LLM-powered agents: Examiner, Questioner, and Assessor. The collaboration among these three agents is designed to realize comprehensive and in-depth weakness identification. Our framework demonstrates significant success in uncovering flaws, with an identification success rate exceeding 30% in prominent models such as ChatGPT and Claude. More importantly, these identified weaknesses can guide specific model improvements, proving more effective than untargeted data augmentation methods like Self-Instruct. Our approach has led to substantial enhancements in popular LLMs, including the Llama series and Mistral-7b, boosting their performance by over 10% across several benchmarks. Code and data are publicly available at https://github.com/thu-coai/AutoDetect.

==> sections/abstract_old.tex <==
% 随着大规模语言模型（LLMs）的能力日益增强，准确识别并解决模型存在的问题成为性能优化的关键步骤。然而，现有的基准存在数据泄漏，更新周期长，没有针对性等问题，难以真实全面的反映出一个模型的能力与提升方向，而人工评测又费时费力，且不易扩展。因此，本文提出了一个统一的框架，以在各类任务上进行红队行动，揭示LLMs的潜在问题。我们的框架不仅能够在各类任务上执行红队行动，并在chatgpt上达到超过%的攻击成功率，还能根据红队行动的结果指导LLMs的优化。通过丰富的实验，我们展示了这种通用的攻击方法能够有效地找到模型的问题，并提升模型效果。

% 静态评测，泄漏，没有针对性，很难知道具体问题和improvement，benchamrk不一定全面，可能的问题；之前的工作主要在安全，有问题...；我们提出通用框架；实现system/挑战
% contribution:1. general framework for LLM; 2. 全面的错误分析，证明了效果提升，effective to generate synthetic data; 3. (system)
% case study, 测试集不全面
% 局限，self-evaluation bias

% 能力强，可以完成高阶任务
% 可能有看似简单但容易忽略的case，potential weakness，
% weakness的重要性（参考可控生成motivation）hard不代表easy的掌握
% 不宜trigger（benchmark 静态、没有针对性...），但是可能是重要的，人工cost，coverage
% 难以系统性找到weakness
% contribution，自动全面评估，意想不到的地方fail

% LLM is strong but have weakness
% weakness is important
% discover weakness is hard (manual examination is consuming, automatic rely on benchmarks, not targeted)
% intuitive explanation of how to discover weakness (first determine taxonomy, then explore under each point, and reflect to find new potential points)
% we can effectively find weakness, and more importantly, we can enhance model performance based on these weaknesses
% my experiments

% As the capabilities of large language models (LLMs) continue to grow, comprehensively evaluating their capabilities and identifying potential weaknesses of LLMs become a critical problem.
% However, existing benchmarks have issues such as data leakage, lengthy update cycles, and more importantly a lack of specificity, making it difficult to accurately and comprehensively reflect LLMs' capabilities and directions for further improvement. Manual evaluation, on the other hand, is time-consuming and labor-intensive, which cannot easily scale.
% In this paper, we introduce a unified framework, \model, to automatically expose potential weaknesses of LLMs in various tasks. Our framework not only succeeds in identifying weaknesses across a broad range of tasks and LLMs, achieving an impressive attack success rate \hnote{mentioning attack here sounds abrupt.} on several strong LLMs (over 30\% on ChatGPT and Claude), but also ensures the coverage of discovered vulnerabilities \hnote{In general, weakness is different from vulnerability}.
% Through extensive experiments, we have demonstrated the generality and transferability of \model, which can effectively identify and address the weaknesses of LLMs and lead to significant improvements in model performance. Our code and data is publicly available at \url{}.



% roles解释，讲attack效果好，然后说提升效果好

% 最基本的没有掌握，但是可以做更复杂的

% As the capabilities of Large Language Models (LLMs) continue to grow, they are becoming indispensable tools in a wide range of industries. Despite their impressive performance, these models still suffer from shortcomings. Recognizing and addressing these flaws is not only beneficial, but also critical to their effective and reliable use. However, the journey to reveal these weaknesses is challenging.
% As Large Language Models (LLMs) become increasingly essential across a wide range of industries, they still suffer from shortcomings.
%Large Language Models (LLMs) still exhibit notable weaknesses, even though they have been employed in diverse industries.
% \xnote{maybe ``powerful'' vs. ``weakness''}
Identifying and addressing deficiencies in large language models (LLMs) is critical for their reliable and effective deployment in practice.
Existing methods, such as manual examinations, are costly and not scalable, while automated methods that leverage benchmarks often fail to detect weaknesses in specific models, due to their model-agnostic nature. \hnote{The logic is not very clear: if the model does not perform on such benchmarks, why do we fail to identify the weakness?}
In this paper, we introduce a unified framework, \model, to automatically expose potential weaknesses in LLMs across various tasks. 
Inspired by the educational assessment process that measures students' learning outcome, \model consists of three LLM-powered roles: the Examiner, Questioner, and Assessor. \hnote{Do we want to claim we are somehow agent-based?} 
The collaboration among these three agents ensures the thoroughness and depth of identifying weaknesses. \hnote{I think it is not to ensure anything, but realize our specific goal, e.g., maximize diversity.}
Our framework demonstrates significant success in uncovering flaws, with an identification success rate exceeding 30\% in prominent models such as ChatGPT and Claude.
% \model succeeds in discovering weaknesses across a broad range of tasks and LLMs, achieving an impressive identification success rate on several strong LLMs (over 30\% on ChatGPT and Claude). 
% More importantly, these identified weaknesses can guide model enhancements, which is superior to untargeted data augmentation like Self-Instruct, leading to substantial improvements on LLMs by more than 10\% in several benchmarks.
% \xnote{may worth mentioning such ``weakness'' is MORE effective in improving the model compared with ordinary data augmentation like self-instruct.} 
More importantly, these identified weaknesses can guide specific model improvements, proving more effective than untargeted data augmentation methods like Self-Instruct. Our approach has led to substantial enhancements in LLMs, boosting their performance by over 10\% across several benchmarks.
Our code and data is publicly available at \url{}.

==> sections/introduction.tex <==

% 能力强，可以完成高阶任务
% 可能有看似简单但容易忽略的case，potential weakness，
% weakness的重要性（参考可控生成motivation）hard不代表easy的掌握
% 不宜trigger（benchmark 静态、没有针对性...），但是可能是重要的，人工cost，coverage
% 难以系统性找到weakness

% contribution，自动全面评估，意想不到的地方fail

% 阿喀琉斯

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/weakness_detection.pdf}
    \caption{Effective weakness discovery can be a good guide to model enhancement. \model can achieve high attack success rates in the instruction-following, mathematics and coding tasks (A). Moreover, leveraging the attack data, we can further improve LLMs (B).}
    \label{fig:weakness}
    \vspace{-5mm}
\end{figure}

\hnote{``automated weakness detection'' sounds awkward to me.}
With the rapid development of the natural language processing (NLP) field in recent years, large language models (LLMs) have demonstrated excellent performance in diverse tasks \cite{brown2020language, zhang2022opt, zeng2022glm, chowdhery2023palm, touvron2023llama}, suggesting their great potential for real-world applications \cite{ChatGPT, Claude}.
As these LLMs continue to evolve in model sizes and performance, the need for systematically exposing vulnerabilities to ensure their reliability and further guide their improvement becomes increasingly imperative.

% 然而全面、准确的评测模型并不是简单的事情。
% 尽管大模型可能在很多任务，甚至是专业考试上达到了人类水平，它们可能出现很简单的错误，这会很大影响模型的可用性和可靠性。因此，如何全面系统的发现这些问题是非常重要的。
% 现有的方法主要依赖评测基准或人工暴漏。
% 然而评测基准又包括静态和动态，静态评估是没有针对性的，无法针对特定的模型进行针对性的评估，并且由于评测集合的更新周期长，存在数据泄漏，榜单过度饱和的情况。而动态评测基准往往覆盖面不够，难以全面发现问题，

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/framework.pdf}
    \caption{Our framework consists of two cycles, where the outer circulation guarantees the coverage of weakness discovery and the iterative search process guarantees the effectiveness. }
    \label{fig:framework}
    \vspace{-5mm}
\end{figure*}

Nevertheless, conducting a comprehensive and instructive model assessment to discover potential weaknesses is non-trivial. While achieving human-level performance on a wide range of tasks and even professional examinations \cite{achiam2023gpt}, LLMs can still make simple mistakes \hnote{if they are simple mistakes, why are they hard to find?} \cite{ouyang2022training, bubeck2023sparks}. These errors can greatly affect the usability and reliability of the models, making the systematic identification of LLMs' weaknesses crucial. Existing methods for identifying shortcomings predominantly rely on assessment benchmarks and manual examinations. Among these, assessment benchmarks can be categorized into static and dynamic. Static benchmarks \cite{cobbe2021training, srivastava2022beyond, liu2023alignbench} lack specificity, which fail to assess particular models thoroughly. Moreover, they suffer from infrequent updates, data leakage \cite{yang2023rethinking, wei2023skywork}, and leaderboard swamping \cite{guo2023evaluating}, making them unsuitable for targeted evaluation of specific model weaknesses. On the other hand, dynamic benchmarks \cite{bai2024benchmarking} often lack the task coverage and domain adaptability that are necessary to comprehensively uncover all potential issues. Furthermore, for manual examinations, their inherent limitations in scope and scalability prevent them from providing a complete picture of a model's weaknesses.


In this paper, we introduce a pioneering, unified framework designed to systematically expose potential weaknesses within LLMs across a variety of tasks.
As shown in Figure \ref{fig:framework}, \model consists of two loops, taxonomy perfection and iterative search, which guarantee coverage and depth respectively. Specifically, our framework includes three roles: \hnote{it is better to first motivate why we need these three roles, instead of directly listing them}
\begin{itemize}
    \item \textbf{Examiner} is tasked with refining and dynamically enhancing the testing layout, ensuring that the evaluation evolves in response to the changing capabilities and potential vulnerabilities of different LLMs.
    \item \textbf{Questioner} is responsible for creating targeted questions within each assessment point. Through iterative explorations, this agent continually probes for model weaknesses, effectively adapting the line of inquiry to unearth new vulnerabilities as they emerge.
    \item \textbf{Assessor}, informed by the ongoing performance assessments of current models, needs to speculate on potential issues to be incorporated into the testing system, following approval by the examiner to ensure soundness and integrity.
\end{itemize}
The synergistic collaboration among the Examiner, Questioner and Assessor guarantees the thoroughness of the assessment process, while the iterative search by the Questioner ensures the depth of questions adaptable to specific LLMs. With \model, we can systematically conduct automated weakness identification for targeted LLMs.

%%KP: 上述设计无法直接解决前一段提到的现有static / dynamic benchmark和manual examination方法存在的问题
% response: 加了一句话

% 通过大量的实验与评估，我们证明了我们的框架不仅能够在各类任务，包括指令遵循，数学，代码以及传统的安全上实现有效的红队行动，在多个模型上达到了超过50%的攻击成功率。同时，利用我们的红队攻击数据，还能帮助模型提升，仅利用不到1k数据可以让Llama模型在指令遵循任务上有10%的性能提升。

Through extensive experiments and evaluations, we demonstrate that \model is able to perform effective weakness exposure across a diverse range of tasks: instruction-following, mathematics, and coding, achieving an impressive attack success rate of over 50\% on multiple models. 
Furthermore, the insights gained from our evaluations have played a pivotal role in the subsequent improvement of these models. Notably, by integrating less than 1,000 samples derived from \model process into fine-tuning open-sourced models, including Mistral and Llama series models, we have witnessed substantial enhancements, i.e., more than 10\% improvements on several benchmarks.

% 我们的贡献可以被总结为：
% 据我们所知，我们首次探索了在多种任务中系统的暴漏模型缺陷，如指令遵从，代码，数学，彰显了在通用任务上进行Red teaming的潜力
% 我们提出的统一的攻击框架实现了非常有效的攻击，并显示出其通用性，在多个模型和各个任务上达到了50%以上的攻击成功率
% 我们的红队攻击框架可以针对性分析各个模型的缺陷，并且利用这些数据可以有效的提升模型效果，仅用少量数据，就可以在多个任务上实现性能提升，特别的，在指令遵从任务上取得超过10%的提升

Our contribution can be summarized as follows:
\begin{itemize}
    \item To the best of our knowledge, we first systematically explore weakness identifications on multiple generic tasks such as instruction-following, mathematics and coding, highlighting the potential of automatic vulnerability assessments on diverse tasks.
    \item \model has demonstrated exceptional adaptability and effectiveness, with a success rate of over 50\% in uncovering vulnerabilities across multiple models and different tasks.
    \item \model allows for targeted analysis of each model's weaknesses. And leveraging data derived from the assessment process, we can effectively enhance model performance, yielding over 10\% improvement on several tasks.
\end{itemize}

==> sections/introduction_old_red_teaming.tex <==
% 静态评测，泄漏，没有针对性，很难知道具体问题和improvement，所以要动态

% 动态benchamrk不一定全面，可能一直找一个问题

% 找毛病的人

% red teaming换名字？
% 写的更大

% 之前的工作主要在安全，有问题...；我们提出通用框架；实现system/挑战
% contribution:1. general framework for LLM; 2. 全面的错误分析，证明了效果提升，effective to generate synthetic data; 3. (system)
% case study, 测试集不全面
% 局限，self-evaluation bias

% 随着近年来NLP领域的快速发展，大规模语言模型（Large Language Models，LLMs）在各类任务上展现出出色的效果，展现出在现实应用中的巨大潜力。
% 然而，随着模型复杂性和规模的增加，如何准确完善的评估模型，并进一步优化其性能，成为了重要的研究挑战。


% 能力强，可以完成高阶任务
% 可能有看似简单但容易忽略的case，potential weakness，
% weakness的重要性（参考可控生成motivation）hard不代表easy的掌握
% 不宜trigger（benchmark 静态、没有针对性...），但是可能是重要的，人工cost，coverage
% 难以系统性找到weakness

% contribution，自动全面评估，意想不到的地方fail

% 阿喀琉斯

With the rapid development of the Natural Language Processing (NLP) field in recent years, large-scale language models (LLMs) have demonstrated excellent performance in diverse tasks \cite{brown2020language, zhang2022opt, zeng2022glm, chowdhery2023palm, touvron2023llama}, indicating their great potential for real-world applications \cite{ChatGPT, Claude}.
As these LLMs continue to evolve in size and performance, the need for comprehensive and accurate evaluations to further guide their optimization becomes increasingly imperative.

% 然而全面、准确的评测模型并不是简单的事情，主要的挑战在于如何科学的构建评测集与评估模型。
% 尽管现在主流的评估数据集都有大量的人工投入，例如引入专业领域的专家进行数据审核，或者采用各类算法来提高数据的多样性和准确性。

Nevertheless, conducting a comprehensive and instructive model assessment is non-trivial. The main challenge lies in how to scientifically construct evaluation datasets. 
Despite the significant efforts invested in the current mainstream evaluation datasets, such as involving human experts for data verification \cite{cobbe2021training, srivastava2022beyond}, or incorporating various algorithms to enhance data diversity and quality \cite{liu2023alignbench, huang2024c}, these benchmarks still suffer from some deficiencies:
\begin{itemize}
    \item \textbf{Data Leakage:}
    % 由于大多评估数据集基本都是静态的，并不会定期更新。因此这些数据集面临很大的泄漏风险，例如可能被用于模型的预训练或微调。这种现象在很多常用的数据集上都有所验证，这大大影响了这些benchmark的可信度。    
    Most evaluation datasets are essentially static and undergo no regular updates, leaving them susceptible to high risk of leakage. For instance, these datasets may be used for pre-training or fine-tuning models \cite{yang2023rethinking, wei2023skywork}, which greatly affects their trustworthiness.
    \item \textbf{Leaderboard Swamping:}
    % 不comprehensive，很快过拟合
    % 随着模型的进步，各方面的能力飞速进步，而大部分评估集合无法全面的覆盖所有类型，这会导致这些benchmark很快被过度拟合而过时。
    As LLMs advance, their capabilities across various aspects are progressing rapidly. However, the majority of existing benchmarks fail to offer a holistic evaluation of all types, and their static nature can lead to swift overfitting and obsolescence.
    \item \textbf{Limited Guidance:}
    % 没有针对性
    % 评估数据集往往不会针对模型进行设计，这可能导致这些基准无法很好的针对某个进行评估，难以指导或帮助开发者提升模型。
    Existing benchmarks are usually model-agnostic and weakly targeted, thereby failing to offer actionable guidance for developers to improve their models.
\end{itemize}

% 在安全领域，红队攻击是一种被广泛应用的策略，用于揭示系统的潜在弱点。通过模拟对手的攻击行为，红队行动旨在找出系统的漏洞，并提供改进的建议。然而，尽管这种策略在安全领域被证明是有效的，但其在通用任务，特别是大规模语言模型中的应用却相对有限。

The strategy of \textit{Red Teaming}, traditionally employed in the security field to reveal potential issues \cite{perez2022red}, offers one promising solution.
Red teaming aims to provide a comprehensive and dynamic assessment, capable of identifying vulnerabilities, and providing guidance for improvement. 
Nevertheless, although its effectiveness is well-demonstrated in the security domain \cite{perez2022red, ganguli2022red, hong2024curiosity}, the application to general-purpose tasks, particularly within the scope of LLMs, remains unexplored.


% 因此，我们提出了一种新的、统一的框架，利用红队行动的策略，来揭示和解决大规模语言模型在各类任务中可能存在的问题。如图1所示，我们的框架共包括三种大模型的agent，组成了两种循环体系。其中，主考官负责细化和动态完善考点体系，出题人负责在每个考点下出题，并进行迭代搜索，来不断找到模型的缺陷，评估者需要根据当前模型的表现推测出新的问题，并经过主考官的审核加入考点体系。其中，主考官，出题人和评估者的循环保证了评估的完善性，而出题人的迭代搜索保证了出题的深度。

In this paper, we propose a novel, unified framework that leverages the \textit{Red Teaming} strategy, aiming to expose potential weaknesses within LLMs across various tasks beyond safety.
As shown in Figure 1, our proposed framework consists of three LLM-powered agents, each undertaking specific roles: 1) \textit{Examiner} is tasked with refining and dynamically enhancing the test layout; 2) \textit{Question Setter} is responsible for creating targeted questions within each test point with iterative explorations, aiming at continually identifying model weaknesses; 3) \textit{Evaluator} needs to speculate potential issues informed by the performance of current models to be incorporated into the test system, following approval by the examiner. The circular collaboration between the examiner, question setter and evaluator ensures the comprehensiveness of the assessment process, while the iterative search by the question setter ensures the depth of questions.

% 通过大量的实验与评估，我们证明了我们的框架不仅能够在各类任务，包括指令遵循，数学，代码以及传统的安全上实现有效的红队行动，在多个模型上达到了超过50%的攻击成功率。同时，利用我们的红队攻击数据，还能帮助模型提升，仅利用不到1k数据可以让Llama模型在指令遵循任务上有10%的性能提升。

Through extensive experiments and evaluations, we demonstrate that our framework is able to perform effective red-teaming evaluation across a diverse range of tasks, including instruction-following, math, and coding, achieving an impressive attack success rate of over 50\% on multiple models. 
Moreover, leveraging our red-team attack data has greatly contributed to the improvement of these models. Remarkably, when fine-tuning Llama models with less than 1k red teaming samples, we have observed more than a 10\% improvement on IFEval \cite{zhou2023instruction} and GSM8k \cite{cobbe2021training} datasets.

% 我们的贡献可以被总结为：
% 据我们所知，我们首次探索了红队攻击被应用于多种通用任务，如指令遵从，代码，数学，彰显了在通用任务上进行Red teaming的潜力
% 我们提出的统一的攻击框架实现了非常有效的攻击，并显示出其通用性，在多个模型和各个任务上达到了50%以上的攻击成功率
% 我们的红队攻击框架可以针对性分析各个模型的缺陷，并且利用这些数据可以有效的提升模型效果，仅用少量数据，就可以在多个任务上实现性能提升，特别的，在指令遵从任务上取得超过10%的提升

Our contribution can be summarized as follows:
\begin{itemize}
    \item To the best of our knowledge, we first explore applying red teaming attacks to multiple generic tasks such as instruction-following, code, and math, highlighting the potential of red teaming on diverse tasks beyond safety.
    \item Our proposed unified red teaming framework has proven effective and adaptable, achieving more than a 50\% attack success rate on multiple models across various tasks.
    \item Our framework allows for targeted analysis of each model's weaknesses. By leveraging red-team data, we can effectively enhance model performance, yielding over 10\% improvement on several tasks.
\end{itemize}

==> tables/improvement.tex <==
\begin{table*}[!t]
    \centering
    \setlength{\tabcolsep}{1mm}
    % \scalebox{1}[0.9]{
    \resizebox{0.85\linewidth}{!}{
        \begin{tabular}{cc|ll|ll|l}
            \toprule
            \multicolumn{2}{l|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c|}{\textbf{Instruction following}} & \multicolumn{2}{c|}{\textbf{Mathematics}} & \multicolumn{1}{c}{\textbf{Coding}} \\ % \cmidrule(l){3-7} 
            \multicolumn{2}{c|}{} & \multicolumn{1}{c}{\textbf{IFEval-p}} & \multicolumn{1}{c|}{\hspace{-0.2em}\textbf{IFEval-i}} & \multicolumn{1}{c}{\hspace{-1em}\textbf{GSM8k}} & \multicolumn{1}{c|}{\hspace{-1em}\textbf{MATH}} & \multicolumn{1}{c}{\textbf{HumanEval}} \\ \midrule
            \multicolumn{1}{l}{\multirow{2}{*}{Llama2-7b-Chat}} & ori. & \hspace{1.2em}32.3 & \hspace{1.5em}46.2 & \hspace{1.2em}18.9 & \hspace{1em}2.5 & \hspace{2em}13.4 \\ 
            \multicolumn{1}{c}{} & ours & \hspace{1.2em}42.5 {\color{ForestGreen} \textsubscript{\textbf{(+10.2)}}} & \hspace{1.5em}54.7 {\color{ForestGreen} \textsubscript{\textbf{(+8.5)}}} & \hspace{1.2em}25.9 {\color{ForestGreen} \textsubscript{\textbf{(+7.0)}}} & \hspace{1em}4.7 {\color{ForestGreen} \textsubscript{\textbf{(+2.2)}}} & \hspace{2em}18.7 {\color{ForestGreen} \textsubscript{\textbf{(+5.3)}}} \\ \midrule
            \multicolumn{1}{l}{\multirow{2}{*}{Llama2-13b-Chat}} & ori. & \hspace{1.2em}34.3 & \hspace{1.5em}45.8 & \hspace{1.2em}26.9 & \hspace{1em}3.9 & \hspace{2em}17.7 \\
            \multicolumn{1}{c}{} & ours & \hspace{1.2em}43.3 {\color{ForestGreen} \textsubscript{\textbf{(+9.0)}}} & \hspace{1.5em}54.3 {\color{ForestGreen} \textsubscript{\textbf{(+8.5)}}} & \hspace{1.2em}33.7 {\color{ForestGreen} \textsubscript{\textbf{(+6.8)}}} & \hspace{1em}6.0 {\color{ForestGreen} \textsubscript{\textbf{(+2.1)}}} & \hspace{2em}24.4 {\color{ForestGreen} \textsubscript{\textbf{(+6.7)}}} \\ \midrule
            \multicolumn{1}{l}{\multirow{2}{*}{Llama2-70b-Chat}} & ori. & \hspace{1.2em}44.2 & \hspace{1.5em}54.3 & \hspace{1.2em}51.9 & \hspace{1em}6.5 & \hspace{2em}31.7 \\
            \multicolumn{1}{c}{} & ours & \hspace{1.2em}51.8 {\color{ForestGreen} \textsubscript{\textbf{(+7.6)}}} & \hspace{1.5em}63.5 {\color{ForestGreen} \textsubscript{\textbf{(+9.2)}}} & \hspace{1.2em}65.0 {\color{ForestGreen} \textsubscript{\textbf{(+13.1)}}} & \hspace{1em}12.6 {\color{ForestGreen} \textsubscript{\textbf{(+6.1)}}} & \hspace{2em}36.6 {\color{ForestGreen} \textsubscript{\textbf{(+4.9)}}} \\ \midrule
            \multicolumn{1}{l}{\multirow{2}{*}{Mistral-7b-Instruct}} & ori. & \hspace{1.2em}51.2 & \hspace{1.5em}61.6 & \hspace{1.2em}42.9 & \hspace{1em}4.5 & \hspace{2em}32.9 \\    
            \multicolumn{1}{c}{} & ours & \hspace{1.2em}54.3 {\color{ForestGreen} \textsubscript{\textbf{(+3.1)}}} & \hspace{1.5em}64.7 {\color{ForestGreen} \textsubscript{\textbf{(+3.1)}}} & \hspace{1.2em}54.8 {\color{ForestGreen} \textsubscript{\textbf{(+11.9)}}} & \hspace{1em}12.6 {\color{ForestGreen} \textsubscript{\textbf{(+8.1)}}} & \hspace{2em}40.9 {\color{ForestGreen} \textsubscript{\textbf{(+8.0)}}} \\ \midrule
            \multicolumn{1}{l}{\multirow{2}{*}{Llama3-8b-Instruct}} & ori. & \hspace{1.2em}70.1 & \hspace{1.5em}78.3 & \hspace{1.2em}75.4 & \hspace{1em}23.9 & \hspace{2em}55.5 \\    
            \multicolumn{1}{c}{} & ours & \hspace{1.2em}72.6 {\color{ForestGreen} \textsubscript{\textbf{(+2.5)}}} & \hspace{1.5em}79.7 {\color{ForestGreen} \textsubscript{\textbf{(+1.4)}}} & \hspace{1.2em}79.9 {\color{ForestGreen} \textsubscript{\textbf{(+4.5)}}} & \hspace{1em}27.1 {\color{ForestGreen} \textsubscript{\textbf{(+3.2)}}} & \hspace{2em}61.0 {\color{ForestGreen} \textsubscript{\textbf{(+5.5)}}} \\ 
            \bottomrule
        \end{tabular}
    }
    \caption{LLMs' performance on different benchmarks of three fundamental tasks before and after training with data derived from the identification process. We use Prompt-level and Inst-level metrics in strict-accuracy for the evaluation of IFEval benchmark (denoted as IFEval-p and IFEval-i respectively).}
    \label{tab:improvement}
    %%%hml：这些指标，距离最强的开源模型多远？
    % response: 目前最强的开源模型都是刷榜的结果，大部分是在同分布数据上微调得到的，比如在metamath上训练后的模型在gsm8k和MATH上就会很高，但是我们的方法并不会利用测试集的信息，所以分布差距比较大，对比并不公平
    \vspace{-3mm}
\end{table*}

==> tables/improvement_v3.tex <==
\begin{table*}[!t]
    \centering
    % \small
    \setlength{\tabcolsep}{1mm}
    % \scalebox{1}[0.9]{
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|cccccc|cccccc|ccc}
            \toprule
            \multicolumn{1}{l|}{\multirow{3}{*}{\textbf{Model}}} & \multicolumn{6}{c|}{\textbf{Instruction following}} & \multicolumn{6}{c|}{\textbf{Mathematics}} & \multicolumn{3}{c}{\textbf{Coding}} \\ % \cmidrule(l){3-7} 
            \multicolumn{1}{c|}{} & \multicolumn{3}{c}{\textbf{IFEval-p}} & \multicolumn{3}{c|}{\textbf{IFEval-i}} & \multicolumn{3}{c}{\textbf{GSM8k}} & \multicolumn{3}{c|}{\textbf{MATH}} & \multicolumn{3}{c}{\textbf{HumanEval}} \\

            \multicolumn{1}{c|}{} & \multicolumn{1}{c}{ori.} & \multicolumn{1}{c}{ours} & \multicolumn{1}{c}{imp.} & \multicolumn{1}{c}{ori.} & \multicolumn{1}{c}{ours} & \multicolumn{1}{c|}{imp.} & \multicolumn{1}{c}{ori.} & \multicolumn{1}{c}{ours} & \multicolumn{1}{c}{imp.} & \multicolumn{1}{c}{ori.} & \multicolumn{1}{c}{ours} & \multicolumn{1}{c|}{imp.} & \multicolumn{1}{c}{ori.} & \multicolumn{1}{c}{ours} & \multicolumn{1}{c}{imp.} \\ \midrule
            
            \multicolumn{1}{l|}{Llama2-7b-Chat} & 32.3 & 42.5 & +10.2 & 46.2 & 54.7 & +8.5 & 18.9 & 25.9 & +7.0 & 2.5 & 4.7 & +2.2 & 13.4 & 18.7 & +5.3 \\ 
            \multicolumn{1}{l|}{Llama2-7b-Chat} & 32.3 & 42.5 & +10.2 & 46.2 & 54.7 & +8.5 & 18.9 & 25.9 & +7.0 & 2.5 & 4.7 & +2.2 & 13.4 & 18.7 & +5.3 \\ 
            \multicolumn{1}{l|}{Llama2-7b-Chat} & 32.3 & 42.5 & +10.2 & 46.2 & 54.7 & +8.5 & 18.9 & 25.9 & +7.0 & 2.5 & 4.7 & +2.2 & 13.4 & 18.7 & +5.3 \\ 
            \multicolumn{1}{l|}{Llama2-7b-Chat} & 32.3 & 42.5 & +10.2 & 46.2 & 54.7 & +8.5 & 18.9 & 25.9 & +7.0 & 2.5 & 4.7 & +2.2 & 13.4 & 18.7 & +5.3 \\ 
            \multicolumn{1}{l|}{Llama2-7b-Chat} & 32.3 & 42.5 & +10.2 & 46.2 & 54.7 & +8.5 & 18.9 & 25.9 & +7.0 & 2.5 & 4.7 & +2.2 & 13.4 & 18.7 & +5.3 \\ 
            \bottomrule
        \end{tabular}
    }
    \caption{LLMs' performance on different benchmarks of three fundamental tasks before and after training with data derived from the identification process. We use Prompt-level and Inst-level metrics in strict-accuracy for the evaluation of IFEval benchmark (denoted as IFEval-p and IFEval-i respectively).}
    \label{tab:improvement}
    %%%hml：这些指标，距离最强的开源模型多远？
    % response: 目前最强的开源模型都是刷榜的结果，大部分是在同分布数据上微调得到的，比如在metamath上训练后的模型在gsm8k和MATH上就会很高，但是我们的方法并不会利用测试集的信息，所以分布差距比较大，对比并不公平
    \vspace{-3mm}
\end{table*}

==> tables/main_results.tex <==
% 有点空，信息量略少，加个列？（seed和迭代的分数）

\begin{table*}[!t]
    \centering
    \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{c|cc|cc|cc}
        \toprule
        \multirow{2}{*}{Model} & \multicolumn{2}{c|}{Instruction Following} & \multicolumn{2}{c|}{Mathematics} & \multicolumn{2}{c}{Coding} \\ 
         & ASR (\%) & Avg. score & ASR (\%) & Avg. score & ASR (\%) & Avg. score \\ \midrule
        Llama2-7b-Chat & 43.33 & 4.66 & 88.79 & 1.99 & 74.76 & 3.06 \\
        Llama2-13b-Chat & 39.72 & 4.75 & 86.07 & 2.31 & 67.46 & 3.57 \\
        Llama2-70b-Chat & 37.33 & 5.04 & 76.85 & 3.06 & 59.84 & 4.17 \\
        Mistral-7b-Chat & 38.19 & 4.87 & 74.07 & 3.27 & 52.06 & 4.77 \\ \midrule
        GPT-3.5 & 25.51 & 5.81 & 50.19 & 5.24 & 32.45 & 6.24 \\
        Mistral-large & 20.29 & 6.40 & 33.89 & 6.71 & 26.35 & 6.55 \\
        Claude-3-sonnet & 19.17 & 6.24 & 43.77 & 5.90 & 29.91 & 6.49 \\ \bottomrule
        \end{tabular}
    }
    \label{tab:mainres}
\end{table*}
